Graph theoretic proofs for some results on banded inverses of $M$-matrices

This work concerns results on conditions guaranteeing that certain banded $M$-matrices have banded inverses. As a first goal, a graph theoretic characterization for an off-diagonal entry of the inverse of an $M$-matrix to be positive, is presented. This result, in turn, is used in providing alternative graph theoretic proofs of the following: (1) a characterization for a tridiagonal $M$-matrix to have a tridiagonal inverse. (2) a necessary condition for an $M$-matrix to have a pentadiagonal inverse. The results are illustrated by several numerical examples.

==> tfcad.bst.tex <==
%%
%% This is file `tfcad.bst',
%% generated with the docstrip utility,
%% modified by DjL 2017/04/18
%% -------------------------------------
%%
%% *** BibTeX style for Taylor & Francis Chicago author-date reference style
%% as described at
%% http://www.tandf.co.uk/journals/authors/style/reference/tf_ChicagoAD.pdf ***
%%
% ===================================================================
% IMPORTANT NOTICE:
% This bibliographic style (bst) file has been generated from one or
% more master bibliographic style (mbs) files.
%
% This file can be redistributed and/or modified under the terms
% of the LaTeX Project Public License Distributed from CTAN
% archives in directory macros/latex/base/lppl.txt; either
% version 1 of the License, or any later version.
% ===================================================================
% Name and version information of the main mbs file:
% \ProvidesFile{merlin.mbs}[2011/11/18 4.33 (PWD, AO, DPC)]
%   For use with BibTeX version 0.99a or later
%   Copyright 1994-2011 Patrick W Daly
%--------------------------------------------------------------------
% This bibliography style file is intended for texts in ENGLISH
% This is an author-year citation style bibliography. As such, it is
% non-standard LaTeX, and requires a special package file to function properly.
% Such a package is    natbib.sty   by Patrick W. Daly
% The form of the \bibitem entries is
%  \bibitem[Jones et~al.(1990)]{key}...
% The essential feature is that the label (the part in brackets) consists
% of the author names, as they should appear in the citation, with the year
% in parentheses following. There must be no space before the opening
% parenthesis!
% With natbib v5.3, a full list of authors may also follow the year.
% In natbib.sty, it is possible to define the type of enclosures that is
% really wanted (brackets or parentheses), but in either case, there must
% be parentheses in the label.
% The \cite command functions as follows:
%  \citet{key} ==>>                Jones et al. (1990)
%  \citet[chap.~2]{key} ==>>       Jones et al. (1990, chap. 2)
%  \citep{key} ==>>               (Jones et al. 1990)
%  \citep[chap.~2]{key} ==>>      (Jones et al. 1990, chap. 2)
%  \citep[e.g.][]{key} ==>>       (e.g. Jones et al. 1990)
%  \citep[e.g.][32]{key} ==>>     (e.g. Jones et al. 1990, 32)
%  \citealt{key} ==>>              Jones et al. 1990
%  \citealp{key} ==>>              Jones et al. 1990
%  \citealp[32]{key} ==>>          Jones et al. 1990, 32
%  \citeauthor{key} ==>>           Jones et al.
%  \citeyear{key} ==>>             1990
%  \citeyearpar{key} ==>>         (1990)
%--------------------------------------------------------------------

ENTRY
{ address
	archive
	author
	booktitle
	chapter
	collaboration
	edition
	editor
	eid
	howpublished
	institution
	journal
	key
	lastchecked
	month
	note
	number
	numpages
	organization
	pages
	publisher
	school
	series
	title
	type
	url
	urldate
	volume
	year
}
{}
{ label extra.label sort.label }

INTEGERS { output.state before.all mid.sentence after.sentence after.block }

FUNCTION {init.state.consts}
{ #0 'before.all :=
	#1 'mid.sentence :=
	#2 'after.sentence :=
	#3 'after.block :=
}

STRINGS { s t }

FUNCTION {output.nonnull}
{ 's :=
	output.state mid.sentence =
	{ ", " * write$ }
	{ output.state after.block =
		{ add.period$ " " * write$ }
		{ output.state before.all =
			'write$
			{ add.period$ " " * write$ }
			if$
		}
		if$
		mid.sentence 'output.state :=
	}
	if$
	s
}

FUNCTION {output}
{ duplicate$ empty$
	'pop$
	'output.nonnull
	if$
}

FUNCTION {output.check}
{ 't :=
	duplicate$ empty$
	{ pop$ "empty " t * " in " * cite$ * warning$ }
	'output.nonnull
	if$
}

FUNCTION {fin.entry}
{ add.period$
	write$
	newline$
}

FUNCTION {new.block}
{ output.state before.all =
	'skip$
	{ after.block 'output.state := }
	if$
}

FUNCTION {new.sentence}
{ output.state after.block =
	'skip$
	{ output.state before.all =
		'skip$
		{ after.sentence 'output.state := }
		if$
	}
	if$
}

FUNCTION {add.blank}
{  " " * before.all 'output.state :=
}

FUNCTION {date.block}
{
	skip$
}

FUNCTION {not}
{   { #0 }
	{ #1 }
	if$
}

FUNCTION {and}
{   'skip$
	{ pop$ #0 }
	if$
}

FUNCTION {or}
{   { pop$ #1 }
	'skip$
	if$
}

FUNCTION {non.stop}
{ duplicate$
	"}" * add.period$
#-1 #1 substring$ "." =
}

FUNCTION {new.block.checkb}
{ empty$
swap$ empty$
and
'skip$
'new.block
if$
}

FUNCTION {field.or.null}
{ duplicate$ empty$
{ pop$ "" }
'skip$
if$
}

FUNCTION {emphasize}
{ duplicate$ empty$
{ pop$ "" }
{ "\emph{" swap$ * "}" * }
if$
}

FUNCTION {tie.or.space.prefix}
{ duplicate$ text.length$ #3 <
{ "~" }
{ " " }
if$
swap$
}

FUNCTION {capitalize}
{ "u" change.case$ "t" change.case$ }

FUNCTION {space.word}
{ " " swap$ * " " * }
% Here are the language-specific definitions for explicit words.
% Each function has a name bbl.xxx where xxx is the English word.
% The language selected here is ENGLISH
FUNCTION {bbl.and}
{ "and" }

FUNCTION {bbl.etal}
{ "et~al." }

FUNCTION {bbl.editors}
{ "eds" }

FUNCTION {bbl.editor}
{ "ed." }

FUNCTION {bbl.edby}
{ "edited by" }

FUNCTION {bbl.edition}
{ "ed." }

FUNCTION {bbl.volume}
{ "Vol." }

FUNCTION {bbl.of}
{ "of" }

FUNCTION {bbl.number}
{ "no." }

FUNCTION {bbl.nr}
{ "no." }

FUNCTION {bbl.in}
{ "in" }

FUNCTION {bbl.pages}
{ "" }

FUNCTION {bbl.page}
{ "" }

FUNCTION {bbl.eidpp}
{ "pages" }

FUNCTION {bbl.chapter}
{ "chap." }

FUNCTION {bbl.techrep}
{ "Technical {R}eport" }

FUNCTION {bbl.mthesis}
{ "Master's thesis" }

FUNCTION {bbl.phdthesis}
{ "PhD diss." }

FUNCTION {bbl.first}
{ "1st" }

FUNCTION {bbl.second}
{ "2nd" }

FUNCTION {bbl.third}
{ "3rd" }

FUNCTION {bbl.fourth}
{ "4th" }

FUNCTION {bbl.fifth}
{ "5th" }

FUNCTION {bbl.st}
{ "st" }

FUNCTION {bbl.nd}
{ "nd" }

FUNCTION {bbl.rd}
{ "rd" }

FUNCTION {bbl.th}
{ "th" }

MACRO {jan} {"Jan."}
MACRO {feb} {"Feb."}
MACRO {mar} {"Mar."}
MACRO {apr} {"Apr."}
MACRO {may} {"May"}
MACRO {jun} {"Jun."}
MACRO {jul} {"Jul."}
MACRO {aug} {"Aug."}
MACRO {sep} {"Sep."}
MACRO {oct} {"Oct."}
MACRO {nov} {"Nov."}
MACRO {dec} {"Dec."}

FUNCTION {eng.ord}
{ duplicate$ "1" swap$ *
#-2 #1 substring$ "1" =
{ bbl.th * }
{ duplicate$ #-1 #1 substring$
	duplicate$ "1" =
	{ pop$ bbl.st * }
	{ duplicate$ "2" =
		{ pop$ bbl.nd * }
		{ "3" =
			{ bbl.rd * }
			{ bbl.th * }
			if$
		}
		if$
	}
	if$
}
if$
}

MACRO {acmcs} {"ACM Computing Surveys"}

MACRO {acta} {"Acta Informatica"}

MACRO {cacm} {"Communications of the ACM"}

MACRO {ibmjrd} {"IBM Journal of Research and Development"}

MACRO {ibmsj} {"IBM Systems Journal"}

MACRO {ieeese} {"IEEE Transactions on Software Engineering"}

MACRO {ieeetc} {"IEEE Transactions on Computers"}

MACRO {ieeetcad}
{"IEEE Transactions on Computer-Aided Design of Integrated Circuits"}

MACRO {ipl} {"Information Processing Letters"}

MACRO {jacm} {"Journal of the ACM"}

MACRO {jcss} {"Journal of Computer and System Sciences"}

MACRO {scp} {"Science of Computer Programming"}

MACRO {sicomp} {"SIAM Journal on Computing"}

MACRO {tocs} {"ACM Transactions on Computer Systems"}

MACRO {tods} {"ACM Transactions on Database Systems"}

MACRO {tog} {"ACM Transactions on Graphics"}

MACRO {toms} {"ACM Transactions on Mathematical Software"}

MACRO {toois} {"ACM Transactions on Office Information Systems"}

MACRO {toplas} {"ACM Transactions on Programming Languages and Systems"}

MACRO {tcs} {"Theoretical Computer Science"}

FUNCTION {bibinfo.check}
{ swap$
duplicate$ missing$
{
	pop$ pop$
	""
}
{ duplicate$ empty$
	{
		swap$ pop$
	}
	{ swap$
		pop$
	}
	if$
}
if$
}

FUNCTION {bibinfo.warn}
{ swap$
duplicate$ missing$
{
	swap$ "missing " swap$ * " in " * cite$ * warning$ pop$
	""
}
{ duplicate$ empty$
	{
		swap$ "empty " swap$ * " in " * cite$ * warning$
	}
	{ swap$
		pop$
	}
	if$
}
if$
}

FUNCTION {urldate.check}
{ lastchecked empty$
{ urldate empty$
	{ "" }   %   'skip$
	{ "Accessed " urldate * add.period$ }
	if$
}
{ "Accessed " lastchecked * add.period$ }
if$
}

FUNCTION {format.url}
{ url duplicate$ empty$
{ pop$ "" }
{ urldate.check " \urlprefix\url{" * swap$ * "}" * }
if$
}

INTEGERS { nameptr namesleft numnames }

STRINGS  { bibinfo }

FUNCTION {format.names}% as they appear in the list
{ 'bibinfo :=
duplicate$ empty$ 'skip$ {
	's :=
	"" 't :=
	#1 'nameptr :=
	s num.names$ 'numnames :=
	numnames 'namesleft :=
	{ namesleft #0 > }
	{ s nameptr
		duplicate$ #1 >
		{ "{ff~}{vv~}{ll}{, jj}" }
		{ "{vv~}{ll}{, ff}{, jj}" }
		if$
		format.name$
		bibinfo bibinfo.check
		't :=
		nameptr #1 >
		{
			nameptr #7
			#1 + =
			numnames #0
			#10 +
			> and
			{ "others" 't :=
				#1 'namesleft := }
			'skip$
			if$
			namesleft #1 >
			{ ", " * t * }
			{
				s nameptr "{ll}" format.name$ duplicate$ "others" =
				{ 't := }
				{ pop$ }
				if$
				"," *
				t "others" =
				{
					" " * bbl.etal *
				}
				{
					bbl.and
					space.word * t *
				}
				if$
			}
			if$
		}
		't
		if$
		nameptr #1 + 'nameptr :=
		namesleft #1 - 'namesleft :=
	}
	while$
} if$
}

FUNCTION {format.names.ed}
{ 'bibinfo :=
duplicate$ empty$ 'skip$ {
	's :=
	"" 't :=
	#1 'nameptr :=
	s num.names$ 'numnames :=
	numnames 'namesleft :=
	{ namesleft #0 > }
	{ s nameptr
		"{ff~}{vv~}{ll}{, jj}"
		format.name$
		bibinfo bibinfo.check
		't :=
		nameptr #1 >
		{
			namesleft #1 >
			{ ", " * t * }
			{
				s nameptr "{ll}" format.name$ duplicate$ "others" =
				{ 't := }
				{ pop$ }
				if$
				numnames #2 >
				{ "," * }
				'skip$
				if$
				t "others" =
				{
					" " * bbl.etal *
				}
				{
					bbl.and
					space.word * t *
				}
				if$
			}
			if$
		}
		't
		if$
		nameptr #1 + 'nameptr :=
		namesleft #1 - 'namesleft :=
	}
	while$
} if$
}

FUNCTION {format.key}
{ empty$
{ key field.or.null }
{ "" }
if$
}

FUNCTION {format.authors}
{ author "author" format.names
duplicate$ empty$ 'skip$
{ collaboration "collaboration" bibinfo.check
	duplicate$ empty$ 'skip$
	{ " (" swap$ * ")" * }
	if$
	*
}
if$
}

FUNCTION {get.bbl.editor}
{ editor num.names$ #1 > 'bbl.editors 'bbl.editor if$ }

FUNCTION {format.editors}
{ editor "editor" format.names duplicate$ empty$ 'skip$
{
	"," *
	" " *
	get.bbl.editor % capitalize
	%   "(" swap$ * ")" *
	*
}
if$
}

FUNCTION {format.note}
{ note empty$
{ "" }
{ note #1 #1 substring$
	duplicate$ "{" =
		'skip$
		{ output.state mid.sentence =
			{ "l" }
			{ "u" }
			if$
			change.case$
		}
		if$
		note #2 global.max$ substring$ * "note" bibinfo.check
	}
	if$
}

FUNCTION {format.title}
{ title "title" bibinfo.check
	duplicate$ empty$ 'skip$
	{
		"``" swap$ *
		add.period$ "'' " *
	}
	if$
}

FUNCTION {format.btitle}
{ title "title" bibinfo.check
	duplicate$ empty$ 'skip$
	{
		emphasize
	}
	if$
}

FUNCTION {end.quote.title}
{ title empty$
	'skip$
	{ before.all 'output.state := }
	if$
}

FUNCTION {end.quote.btitle}
{ booktitle empty$
	'skip$
	{ editor empty$
		{ before.all 'output.state := }
		'skip$
		if$
	}
	if$
}

FUNCTION {output.bibitem}%
{ newline$
	"\bibitem[" write$
	label write$
	"]{" write$
		cite$ write$
		"}" write$
	newline$
	""
	before.all 'output.state :=
}

FUNCTION {n.dashify}
{ 't :=
	""
	{ t empty$ not }
	{ t #1 #1 substring$ "-" =
		{ t #1 #2 substring$ "--" = not
			{ "--" *
				t #2 global.max$ substring$ 't :=
			}
			{   { t #1 #1 substring$ "-" = }
				{ "-" *
					t #2 global.max$ substring$ 't :=
				}
				while$
			}
			if$
		}
		{ t #1 #1 substring$ *
			t #2 global.max$ substring$ 't :=
		}
		if$
	}
	while$
}

FUNCTION {word.in}
{ bbl.in capitalize
	" " * }

FUNCTION {format.date}
{ year "year" bibinfo.check duplicate$ empty$
	{
		"empty year in " cite$ * "; set to n.d." * warning$
		pop$ "n.d."
	}
	'skip$
	if$
	extra.label *
	before.all 'output.state :=
	after.sentence 'output.state :=
}

FUNCTION {either.or.check}
{ empty$
	'pop$
	{ "can't use both " swap$ * " fields in " * cite$ * warning$ }
	if$
}

FUNCTION {format.bvolume}
{ volume empty$
	{ " " }
	{ bbl.volume volume tie.or.space.prefix
		"volume" bibinfo.check * *
		series "series" bibinfo.check
		duplicate$ empty$ 'pop$
		{ swap$ bbl.of space.word * swap$
			emphasize * }
		if$
		"volume and number" number either.or.check
	}
	if$
}

FUNCTION {format.number.series}
{ volume empty$
	{ number empty$
		{ series field.or.null }
		{ output.state mid.sentence =
			{ "" }
			{ "" }
			if$
			series empty$
			{ "there's a number but no series in " cite$ * warning$ }
			{ series "series" bibinfo.check *
				number tie.or.space.prefix "number" bibinfo.check * * }
			if$
		}
		if$
	}
	{ "" }
	if$
}

FUNCTION {is.num}
{ chr.to.int$
	duplicate$ "0" chr.to.int$ < not
	swap$ "9" chr.to.int$ > not and
}

FUNCTION {extract.num}
{ duplicate$ 't :=
	"" 's :=
	{ t empty$ not }
	{ t #1 #1 substring$
		t #2 global.max$ substring$ 't :=
		duplicate$ is.num
		{ s swap$ * 's := }
		{ pop$ "" 't := }
		if$
	}
	while$
	s empty$
	'skip$
	{ pop$ s }
	if$
}

FUNCTION {convert.edition}
{ extract.num "l" change.case$ 's :=
	s "first" = s "1" = or
	{ bbl.first 't := }
	{ s "second" = s "2" = or
		{ bbl.second 't := }
		{ s "third" = s "3" = or
			{ bbl.third 't := }
			{ s "fourth" = s "4" = or
				{ bbl.fourth 't := }
				{ s "fifth" = s "5" = or
					{ bbl.fifth 't := }
					{ s #1 #1 substring$ is.num
						{ s eng.ord 't := }
						{ edition 't := }
						if$
					}
					if$
				}
				if$
			}
			if$
		}
		if$
	}
	if$
	t
}

FUNCTION {format.edition}
{ edition duplicate$ empty$ 'skip$
	{
		convert.edition
		output.state mid.sentence =
		{ "l" }
		{ "t" }
		if$ change.case$
		"edition" bibinfo.check
		" " * bbl.edition *
	}
	if$
}

INTEGERS { multiresult }

FUNCTION {multi.page.check}
{ 't :=
	#0 'multiresult :=
	{ multiresult not
		t empty$ not
		and
	}
	{ t #1 #1 substring$
		duplicate$ "-" =
		swap$ duplicate$ "," =
		swap$ "+" =
		or or
		{ #1 'multiresult := }
		{ t #2 global.max$ substring$ 't := }
		if$
	}
	while$
	multiresult
}

FUNCTION {format.pages}
{ pages duplicate$ empty$ 'skip$
	{ duplicate$ multi.page.check
		{
			n.dashify
		}
		{
		}
		if$
		"pages" bibinfo.check
	}
	if$
}

FUNCTION {format.journal.pages}
{ pages duplicate$ empty$ 'pop$
	{ swap$ duplicate$ empty$
		{ pop$ pop$ format.pages }
		{
			": " *
			swap$
			n.dashify
			"pages" bibinfo.check
			*
		}
		if$
	}
	if$
}

FUNCTION {format.journal.eid}
{ eid "eid" bibinfo.check
	duplicate$ empty$ 'pop$
	{ swap$ duplicate$ empty$ 'skip$
		{
			", " *
		}
		if$
		swap$ *
		numpages empty$ 'skip$
		{ bbl.eidpp numpages tie.or.space.prefix
			"numpages" bibinfo.check * *
			" (" swap$ * ")" * *
		}
		if$
	}
	if$
}

FUNCTION {format.vol.num.pages}
{ volume field.or.null
	duplicate$ empty$ 'skip$
	{
	}
	if$
	number "number" bibinfo.check duplicate$ empty$ 'skip$
	{
		swap$ duplicate$ empty$
		{ "there's a number but no volume in " cite$ * warning$ }%%% Chicago would like this to output like , no. 25: without parentheses (CMS 806-7)
		'skip$
		if$
		swap$
		" (" swap$ * ")" *
	}
	if$ *
	eid empty$
	{ format.journal.pages }
	{ format.journal.eid }
	if$
}

FUNCTION {format.chapter.pages}
{ chapter empty$
	'format.pages
	{ type empty$
		{ bbl.chapter capitalize }   %   { bbl.chapter }
		{ type "l" change.case$
			"type" bibinfo.check
		}
		if$
		chapter tie.or.space.prefix
		"chapter" bibinfo.check
		* *
		pages empty$
		'skip$
		{ ", " * format.pages * }
		if$
	}
	if$
}

FUNCTION {bt.emph}
{ duplicate$ empty$ 'skip$
	{ "\emph{" swap$ *
			non.stop
			{ "}, " * }
		{ "}, " * }
	if$
}
if$
}

FUNCTION {format.booktitle}
{
booktitle "booktitle" bibinfo.check
bt.emph
}

FUNCTION {format.in.ed.booktitle}
{ format.booktitle duplicate$ empty$ 'skip$
{ editor "editor" format.names.ed duplicate$ empty$ 'pop$
	{ bbl.edby
		" " * swap$ *
		swap$
		" " * swap$
		* }
	if$
	word.in swap$ *
}
if$
}

FUNCTION {empty.misc.check}%
{ author empty$ title empty$ howpublished empty$
month empty$ year empty$ note empty$
and and and and and
key empty$ not and
{ "all relevant fields are empty in " cite$ * warning$ }
'skip$
if$
}

FUNCTION {format.thesis.type}
{ type duplicate$ empty$
'pop$
{ swap$ pop$
	%      "t" change.case$
	"type" bibinfo.check
}
if$
}

FUNCTION {format.tr.number}
{ number "number" bibinfo.check
type duplicate$ empty$
{ pop$ bbl.techrep }
'skip$
if$
"type" bibinfo.check
swap$ duplicate$ empty$
{ pop$ "t" change.case$ }
{ tie.or.space.prefix * * }
if$
}

FUNCTION {format.article.crossref}
{
word.in
" \cite{" * crossref * "}" *
}

FUNCTION {format.book.crossref}
{ volume duplicate$ empty$
{ "empty volume in " cite$ * "'s crossref of " * crossref * warning$
	pop$ word.in
}
{ bbl.volume
	swap$ tie.or.space.prefix "volume" bibinfo.check * * bbl.of space.word *
}
if$
" \cite{" * crossref * "}" *
}

FUNCTION {format.incoll.inproc.crossref}
{
word.in
" \citealt{" * crossref * "}" *
}

FUNCTION {format.org.or.pub}
{ 't :=
""
address empty$ t empty$ and
'skip$
{
	address "address" bibinfo.check *
	t empty$
	'skip$
	{ address empty$
		'skip$
		{ ": " * }
		if$
		t *
	}
	if$
}
if$
}

FUNCTION {format.publisher.address}
{ publisher "publisher" bibinfo.warn format.org.or.pub
}

FUNCTION {format.organization.address}
{ organization "organization" bibinfo.check format.org.or.pub
}

FUNCTION {format.institution.address}
{ institution "institution" bibinfo.warn format.org.or.pub
}

FUNCTION {format.address}
{ address empty$
{ "" }
{ address "address" bibinfo.check}
if$
}

FUNCTION {format.month}
{ month empty$
{ "" }
{ month "month" bibinfo.check
	"" swap$ * "" *}
if$
}

FUNCTION {article}
{ output.bibitem
format.authors "author" output.check
author format.key output
format.date "year" output.check
new.block
format.title "title" output.check
end.quote.title
crossref missing$
{
	journal
	"journal" bibinfo.check
	emphasize
	"journal" output.check
	add.blank
	format.vol.num.pages output
}
{ format.article.crossref output.nonnull
	format.pages output
}
if$
new.block
format.note output
format.url output
fin.entry
}

FUNCTION {book}
{ output.bibitem
author empty$
{ format.editors "author and editor" output.check
	editor format.key output
}
{ format.authors output.nonnull
	crossref missing$
	{ "author and editor" editor either.or.check }
	'skip$
	if$
}
if$
format.date "year" output.check
new.block
format.btitle "title" output.check
new.sentence%
crossref missing$
{ format.edition output
	format.bvolume output
	format.number.series output
	new.sentence
	format.publisher.address output
}
{ new.block
	format.book.crossref output.nonnull
}
if$
new.block
format.note output
format.url output
fin.entry
}

FUNCTION {booklet}
{ output.bibitem
format.authors output
author format.key output
format.date "year" output.check
new.block
format.title "title" output.check
end.quote.title
howpublished "howpublished" bibinfo.check output
address "address" bibinfo.check output
new.block
format.note output
format.url output
fin.entry
}

FUNCTION {inbook}
{ output.bibitem
author empty$
{ format.editors "author and editor" output.check
	editor format.key output
}
{ format.authors output.nonnull
	crossref missing$
	{ "author and editor" editor either.or.check }
	'skip$
	if$
}
if$
format.date "year" output.check
new.block
format.btitle "title" output.check
crossref missing$
{ format.edition output
	format.bvolume output
	format.chapter.pages "chapter and pages" output.check
	new.block
	format.number.series output
	new.sentence
	format.publisher.address output
}
{
	format.chapter.pages "chapter and pages" output.check
	new.block
	format.book.crossref output.nonnull
}
if$
new.block
format.note output
format.url output
fin.entry
}

FUNCTION {incollection}
{ output.bibitem
format.authors "author" output.check
author format.key output
format.date "year" output.check
new.block
format.title "title" output.check
end.quote.title
crossref missing$
{ format.in.ed.booktitle "booktitle" output.check
	end.quote.btitle
	format.edition output
	format.bvolume output
	format.number.series output
	format.chapter.pages output
	new.sentence
	format.publisher.address output
}
{ format.incoll.inproc.crossref output.nonnull
	format.chapter.pages output
}
if$
new.block
format.note output
format.url output
fin.entry
}

FUNCTION {inproceedings}
{ output.bibitem
format.authors "author" output.check
author format.key output
format.date "year" output.check
new.block
format.title "title" output.check
end.quote.title
crossref missing$
{ format.in.ed.booktitle "booktitle" output.check
	end.quote.btitle
	format.bvolume output
	format.number.series output
	format.address output
	format.month output
	format.pages output
	new.sentence
	publisher empty$
	{ organization output }
	{ organization "organization" bibinfo.check output
		publisher output
	}
	if$
}
{ format.incoll.inproc.crossref output.nonnull
	format.pages output
}
if$
new.block
format.note output
format.url output
fin.entry
}

FUNCTION {conference} { inproceedings }

FUNCTION {manual}
{ output.bibitem
format.authors output
author format.key output
format.date "year" output.check
new.block
format.btitle "title" output.check
new.sentence
format.edition output
new.sentence
format.organization.address "organization and address" output.check
new.block
format.note output
format.url output
fin.entry
}

FUNCTION {mastersthesis}
{ output.bibitem
format.authors "author" output.check
author format.key output
format.date "year" output.check
new.block
format.title "title" output.check
end.quote.title
bbl.mthesis format.thesis.type output.nonnull
school "school" bibinfo.warn output
address "address" bibinfo.check output
new.block
format.note output
format.url output
fin.entry
}

FUNCTION {misc}
{ output.bibitem
format.authors output
author format.key output
format.date "year" output.check
new.block
format.title output
end.quote.title
howpublished "howpublished" bibinfo.check output
address "address" bibinfo.check output%
format.month output%
new.block
format.note output
format.url output
fin.entry
}

FUNCTION {phdthesis}
{ output.bibitem
format.authors "author" output.check
author format.key output
format.date "year" output.check
new.block
format.title "title" output.check
end.quote.title
bbl.phdthesis format.thesis.type output.nonnull
school "school" bibinfo.warn output
address "address" bibinfo.check output
new.block
format.note output
format.url output
fin.entry
}

FUNCTION {presentation}
{ output.bibitem
format.authors output
author format.key output
format.date "year" output.check
new.block%
format.title output
end.quote.title
organization output
address output
format.month output%
new.sentence
format.note output
new.sentence
type missing$ 'skip$
{"(" type capitalize * ")" * output}
if$
format.url output
fin.entry
}

FUNCTION {proceedings}
{ output.bibitem
editor empty$
{ organization output
	organization format.key output }
{ format.editors output.nonnull }
if$
format.date "year" output.check
new.block
format.btitle "title" output.check
format.bvolume output
format.number.series output
address output
format.month output
new.sentence
organization output
publisher output
new.block
format.note output
format.url output
fin.entry
}

FUNCTION {techreport}
{ output.bibitem
format.authors "author" output.check
author format.key output
format.date "year" output.check
new.block
format.btitle
"title" output.check
new.block
format.tr.number output.nonnull
new.block
format.institution.address output
new.block
format.note output
format.url output
fin.entry
}

FUNCTION {unpublished}
{ output.bibitem
format.authors "author" output.check
author format.key output
format.date "year" output.check
new.block
format.title "title" output.check
end.quote.title
new.block
format.note "note" output.check
format.url output
fin.entry
}

FUNCTION {default.type} { misc }

READ

FUNCTION {sortify}
{ purify$
"l" change.case$
}

INTEGERS { len }

FUNCTION {chop.word}
{ 's :=
'len :=
s #1 len substring$ =
{ s len #1 + global.max$ substring$ }
's
if$
}

FUNCTION {format.lab.names}% as they appear in the text
{'s :=
"" 't :=
#1 'nameptr :=
s num.names$ 'numnames :=
numnames 'namesleft :=
{ namesleft #0 > }
{ s nameptr
	"{vv~}{ll}" format.name$
	't :=
	nameptr #1 >
	{
		nameptr #2 =
		numnames #3 > and
		{ "others" 't :=
			#1 'namesleft := }
		'skip$
		if$
		namesleft #1 >
		{ ", " * t * }
		{
			s nameptr "{ll}" format.name$ duplicate$ "others" =
			{ 't := }
			{ pop$ }
			if$
			t "others" =
			{
				" " * bbl.etal *
			}
			{
				numnames #2 >
				{ "," * }
				'skip$
				if$
				bbl.and
				space.word * t *
			}
			if$
		}
		if$
	}
	't
	if$
	nameptr #1 + 'nameptr :=
	namesleft #1 - 'namesleft :=
}
while$
}

FUNCTION {author.key.label}
{ author empty$
{ key empty$
	{ cite$ #1 #3 substring$ }
	'key
	if$
}
{ author format.lab.names }
if$
}

FUNCTION {author.editor.key.label}
{ author empty$
{ editor empty$
	{ key empty$
		{ cite$ #1 #3 substring$ }
		'key
		if$
	}
	{ editor format.lab.names }
	if$
}
{ author format.lab.names }
if$
}

FUNCTION {editor.key.label}
{ editor empty$
{ key empty$
	{ cite$ #1 #3 substring$ }
	'key
	if$
}
{ editor format.lab.names }
if$
}

FUNCTION {calc.label}
{ type$ "book" =
type$ "inbook" =
or
'author.editor.key.label
{ type$ "proceedings" =
	'editor.key.label
	'author.key.label
	if$
}
if$
"("
*
year duplicate$ empty$
{ pop$ "n.d." }
'skip$
if$
*
'label :=
}

FUNCTION {sort.format.names}
{ 's :=
#1 'nameptr :=
""
s num.names$ 'numnames :=
numnames 'namesleft :=
{ namesleft #0 > }
{ nameptr #1 >
	{ "   " * }
	'skip$
	if$
	s nameptr "{vv{ } }{ll{ }}{  ff{ }}{  jj{ }}" format.name$ 't :=
	nameptr numnames = t "others" = and
	{ bbl.etal * }
	{ t sortify * }
	if$
	nameptr #1 + 'nameptr :=
	namesleft #1 - 'namesleft :=
}
while$
}

FUNCTION {sort.format.title}
{ 't :=
"A " #2
"An " #3
"The " #4 t chop.word
chop.word
chop.word
sortify
#1 global.max$ substring$
}

FUNCTION {author.sort}
{ author empty$
{ key empty$
	{ "to sort, need author or key in " cite$ * warning$
		"" }
	{ key sortify }
	if$
}
{ author sort.format.names }
if$
}

FUNCTION {editor.sort}
{ editor empty$
{ key empty$
	{ "to sort, need editor or key in " cite$ * warning$
		""
	}
	{ key sortify }
	if$
}
{ editor sort.format.names }
if$
}

FUNCTION {author.editor.sort}
{ author empty$
{ editor empty$
	{ key empty$
		{ "to sort, need author, editor, or key in " cite$ * warning$
			""
		}
		{ key sortify }
		if$
	}
	{ editor sort.format.names }
	if$
}
{ author sort.format.names }
if$
}

FUNCTION {presort}
{ calc.label
label sortify
"    "
*
type$ "book" =
type$ "inbook" =
or
'author.editor.sort
{ type$ "proceedings" =
	'editor.sort
	'author.sort
	if$
}
if$
#1 entry.max$ substring$
'sort.label :=
sort.label
*
"    "
*
title field.or.null
sort.format.title
*
#1 entry.max$ substring$
'sort.key$ :=
}

ITERATE {presort}

SORT

STRINGS { last.label next.extra }

INTEGERS { last.extra.num last.extra.num.extended last.extra.num.blank number.label }

FUNCTION {initialize.extra.label.stuff}
{ #0 int.to.chr$ 'last.label :=
"" 'next.extra :=
#0 'last.extra.num :=
"a" chr.to.int$ #1 - 'last.extra.num.blank :=
last.extra.num.blank 'last.extra.num.extended :=
#0 'number.label :=
}

FUNCTION {forward.pass}
{ last.label label =
{ last.extra.num #1 + 'last.extra.num :=
	last.extra.num "z" chr.to.int$ >
	{ "a" chr.to.int$ 'last.extra.num :=
		last.extra.num.extended #1 + 'last.extra.num.extended :=
	}
	'skip$
	if$
	last.extra.num.extended last.extra.num.blank >
	{ last.extra.num.extended int.to.chr$
		last.extra.num int.to.chr$
		* 'extra.label := }
	{ last.extra.num int.to.chr$ 'extra.label := }
	if$
}
{ "a" chr.to.int$ 'last.extra.num :=
	"" 'extra.label :=
	label 'last.label :=
}
if$
number.label #1 + 'number.label :=
}

FUNCTION {reverse.pass}
{ next.extra "b" =
{ "a" 'extra.label := }
'skip$
if$
extra.label 'next.extra :=
extra.label
duplicate$ empty$
'skip$
{ "{\natexlab{" swap$ * "}}" * }
if$
'extra.label :=
label extra.label * ")" * 'label :=
}

EXECUTE {initialize.extra.label.stuff}

ITERATE {forward.pass}

REVERSE {reverse.pass}

FUNCTION {bib.sort.order}
{ sort.label
"    "
*
year field.or.null sortify
*
"    "
*
title field.or.null
sort.format.title
*
#1 entry.max$ substring$
'sort.key$ :=
}

ITERATE {bib.sort.order}

SORT

FUNCTION {begin.bib}
{ preamble$ empty$
'skip$
{ preamble$ write$ newline$ }
if$
"\begin{thebibliography}{" number.label int.to.str$ * "}" *
	write$ newline$
	"\newcommand{\enquote}[1]{``#1''}"
	write$ newline$
	"\providecommand{\natexlab}[1]{#1}"
	write$ newline$
	"\providecommand{\url}[1]{\normalfont{#1}}"
	write$ newline$
	"\providecommand{\urlprefix}{}"
	write$ newline$
}

EXECUTE {begin.bib}

EXECUTE {init.state.consts}

ITERATE {call.type$}

FUNCTION {end.bib}
{ newline$
	"\end{thebibliography}" write$ newline$
}

EXECUTE {end.bib}

%% End of customized bst file
%%
%% End of file `tfcad.bst'.

